Who is more ready to get back in shape?

This empirical study estimates resilience (adaptive capacity) around the periods of the 2013 heavy flood in Cambodia. We use nearly 1.2 million microfinance institution (MFI) customer data and implement the unsupervised learning method. Our results highlight the opportunity to develop resilience by having a better understanding of which areas are likely to be more or less resilient based on the characteristics of the MFI customers, and the individual choices or situations that support stronger adaptiveness. We also discuss the limitation of this approach.

==> tab/tab2.tex <==
\begin{table}
  \caption{Key determinants of clusters at individual level}
  \label{table2}
  \centering
  \begin{tabular}{lll}
    \toprule
    \cmidrule(r){1-2}
    Year     & Determinants   \\  
    \midrule
    2012 & Loan balance, interest rate, loan term  \\
    2013 & Loan balance , local currency, interest rate, loan term, income diversity, schooled \\
    2014 & Loan balance , local currency, interest rate, loan term, age     \\
    2015 & Loan balance , local currency, loan term, age       \\
    \bottomrule
  \end{tabular}
\end{table}
